Diffusion Generative Models in Infinite Dimensions

Diffusion generative models have recently been applied to domains where the available data can be seen as a discretization of an underlying function, such as audio signals or time series. However, these models operate directly on the discretized data, and there are no semantics in the modeling process that relate the observed data to the underlying functional forms. We generalize diffusion models to operate directly in function space by developing the foundational theory for such models in terms of Gaussian measures on Hilbert spaces. A significant benefit of our function space point of view is that it allows us to explicitly specify the space of functions we are working in, leading us to develop methods for diffusion generative modeling in Sobolev spaces. Our approach allows us to perform both unconditional and conditional generation of function-valued data. We demonstrate our methods on several synthetic and real-world benchmarks.

==> scrap/spde_stuff.tex <==
\section{A Stochastic PDE Model}

One way to do this is via a stochastic PDE (SPDE) model. Analogizing with diffusion models in finite-dimensional spaces, we would like to (i) write down an SPDE whose initial distribution is $\P_{\text{data}}$ with a tractable stationary distribution, and (ii) time-reverse this SPDE. 

There are many flavors of SPDEs, but one class that is (relatively) easy to work with is that of \textbf{semilinear SPDEs}. These are defined by equations of the form

\begin{equation}
    \d u_t = L u_t \d t + F(u_t) \d t + G(u_t) \d W_t \qquad u_0 \sim \P_{\text{data}}.
\end{equation}

Here, the collection $\{u_t \}$ should be understood as a sequence in $\hilb$, i.e. for each $t$, we have $u_t = u(t, \blank): \XX \to \YY$ is a function $u_t \in \hilb$. Typically $L$ is a differential operator and $F: \hilb \to \hilb$ is a continuous operator. The mapping $G: \hilb \to \mathcal{L}({\sf{K}}, \hilb)$ outputs a linear operator $Q(u_t): \sf{K} \to \hilb$, where $\mathcal{L}(\sf{K}, \hilb)$ represents the space of linear operators $\sf{K} \to \hilb$. Here, $\sf{K}$ is a second separable Hilbert space on which the infinite-dimensional $Q$-Wiener (or cylindrical) process $W_t$ lives. We let $u_0 \sim \P_{\text{data}}$ be the initial condition of our SPDE, drawn from the data distribution. 

\subsection{Primer on Hilbert Space Wiener Processes}

By a $Q$-Wiener process, we mean that we specify an operator $Q: {\sf{K} \to \sf{K}}$ to obtain an infinite-dimensional analogue of Brownian motion. Under some additional assumptions on $Q$, it turns out that we can write the process $W_t$ as
\begin{equation}
    W(t, x) = \sum \sqrt{\lambda_i} \varphi_i(x) \beta_i (t)
\end{equation}
where $(\lambda_i, \varphi_i)$ are eigentuples for $Q$ and $\beta_i$'s are standard Brownian motions on $\R$, and $\{\varphi_i \}$ forms a complete orthonormal basis for $\sf{K}$. The resulting processes are continuous in $t$. If $Q = \sf{Id}$ is the identity operator, we have for any orthonormal basis $\{\varphi_i \}$ of $\sf{K}$ that
\begin{equation}
    W(t, x) = \sum_i \varphi_i(x) \beta_i(t).
\end{equation}

This is called the \emph{cylindrical} Wiener process. This technically does not converge in $\sf{K}$ but a larger Hilbert space containing $\sf{K}$, but for our purposes we can think of a cylindrical Wiener process as the white noise process.

The operator $Q$ can be thought of as specifying the spatial covariance of our process $W(t, x)$, where the time covariance is obtained via the usual Brownian motion. An informal calculation shows:
\begin{align*}
    \text{Cov}(W(t, x), W(s, y)) &= \E \left[\left(\sum_i \sqrt{\lambda_i} \varphi_i(x) \beta_i (t) \right) \left(\sum_j \sqrt{\lambda_j} \varphi_j(y) \beta_j (s) \right)\right] \\
    &= \sum_{i,j} \sqrt{\lambda_i \lambda_j} \varphi_i (x) \varphi_j(y) \E \left[ \beta_i(t) \beta_j(s) \right] \\
    &= \sum_i \lambda_i \varphi_i(x) \varphi_i(y) \E \left[\beta_i(t) \beta_j(s) \right] \\
    &= (t \wedge s) \sum_i \lambda_i \varphi_i(x) \varphi_i(y).
\end{align*}
Hence the spatial covariance is controlled by $Q$, and time temporal covariance is $t \wedge s$ as expected.



Informally, we can think of an SPDE as an SDE, taking values in some Hilbert space $\hilb$ and driven by some infinite-dimensional Brownian motion $W$. The operators $L, F$ should be interpreted as the drift, and $G$ should be interpreted as the diffusion. Note that $G$ is matrix-valued in the finite-dimensional case, and hence should be operator-valued here. The $\sf{K}$-valued process $W_t$ should be thought of as an infinite-dimensional Brownian motion serving as our source of stochasticity.

If $G$ does not depend on $u_t$ (i.e. is a constant operator), then we say the noise is \textbf{additive}. Otherwise, the noise is \textbf{multiplicative}. If $F \equiv 0$ is identically zero, the semilinear SPDE turns into the special case of a \textbf{linear SPDE}. 

\subsection{Questions}

\begin{itemize}
    \item Let $\P_t \in \PP(\hilb)$ represent the distribution of $u_t$ for any $t \geq 0$. If we set $\P_0 = \P_{\text{data}}$, are there choices of $L, F, G$ such that $\P_t \to \Q$, where $\Q \in \PP(\hilb)$ is some tractable distribution? We at least need to be able to sample from $\Q$. For example, $\Q$ could be a mean-zero Gaussian process with some specified covariance operator $C_\Q$. In the finite-dimensional case, a standard choice is the Ornstein-Uhlenbeck process, but I am not sure an analog exists in the infinite-dimensional setting.
    \item How can we perform time-reversal for an SPDE? One possible route is to see if there are evolution equations (i.e. Kolmogorov equations) for the law $\P_t$, and model ourselves on the proof of the time-reversal in the finite-dimensional case. 
\end{itemize}
